Fully Attentional Networks with Self-emerging Token Labeling

Recent studies indicate that Vision Transformers (ViTs) are robust against out-of-distribution scenarios. In particular, the Fully Attentional Network (FAN) - a family of ViT backbones, has achieved state-of-the-art robustness. In this paper, we revisit the FAN models and improve their pre-training with a self-emerging token labeling (STL) framework. Our method contains a two-stage training framework. Specifically, we first train a FAN token labeler (FAN-TL) to generate semantically meaningful patch token labels, followed by a FAN student model training stage that uses both the token labels and the original class label. With the proposed STL framework, our best model based on FAN-L-Hybrid (77.3M parameters) achieves 84.8% Top-1 accuracy and 42.1% mCE on ImageNet-1K and ImageNet-C, and sets a new state-of-the-art for ImageNet-A (46.1%) and ImageNet-R (56.6%) without using extra data, outperforming the original FAN counterpart by significant margins. The proposed framework also demonstrates significantly enhanced performance on downstream tasks such as semantic segmentation, with up to 1.7% improvement in robustness over the counterpart model. Code is available at https://github.com/NVlabs/STL.

==> Tables/augmentation.tex <==
\begin{table}[htpb]
\centering
\caption{\textbf{Ablation of different data augmentations applied on input images of the token labeler.}}
\label{ablation_agumenation}
\begin{tabular}{c|ccc}
\hline
Spatial &  \cmark    &      &      \\
RandAug &      &      &      \\
CutOut  &      &      &      \\
MixUp   &      &      &      \\
CutMix  &      &      &      \\ \hline
IN-1K   & 83.4 & 82.6 & 83.6 \\
IN-C    & 65.5 & 63.5 & 64.9 \\ \hline
\end{tabular}
\end{table}

==> Tables/comp_diff_tl_training.tex <==
\begin{table}[htbp]
\centering
\small
\begin{tabular}{l|ccc}
Model                  & IN-1K & IN-C & mCE ($\downarrow$) \\ \midrule
FAN-S-Hybrid       &    83.5   &  64.7   &  47.8   \\ \midrule
FAN-TL-S-Hybrid  (sg) &   83.5    &  64.7    &  47.9   \\
STL (FAN-S-Hybrid )  &   83.2    &   65.1   &   47.9  \\ \midrule
FAN-TL-S-Hybrid      &    83.3   &   64.1   &  49.0   \\
STL (FAN-S-Hybrid )  &   83.4    &  \textbf{65.5}    &   \textbf{47.3}  \\ \bottomrule
\end{tabular}
\caption{\textbf{Comparison of different training methods for the token labeler.}}
\label{tl_training}
\end{table}
